CIKAN: Constraint Informed Kolmogorov-Arnold Networks for Autonomous Spacecraft Rendezvous using Time Shift Governor

The paper considers a Constrained-Informed Neural Network (CINN) approximation for the Time Shift Governor (TSG), which is an add-on scheme to the nominal closed-loop system used to enforce constraints by time-shifting the reference trajectory in spacecraft rendezvous applications. We incorporate Kolmogorov-Arnold Networks (KANs), an emerging architecture in the AI community, as a fundamental component of CINN and propose a Constrained-Informed Kolmogorov-Arnold Network (CIKAN)-based approximation for TSG. We demonstrate the effectiveness of the CIKAN-based TSG through simulations of constrained spacecraft rendezvous missions on highly elliptic orbits and present comparisons between CIKANs, MLP-based CINNs, and the conventional TSG.

==> sections/kan.tex <==

\subsection{Structure of KAN}

An activation function of the KAN architecture~\cite{liu2024kan} comprises a basis function and a B-spline function:
\begin{equation} \label{eq:residual_act_fxn}
    \tilde{\phi}(x) =\tilde{\phi}(x ;\theta, \beta, \alpha) = \beta \cdot b(x) + \alpha \cdot {\rm spline}(x; \theta),
\end{equation}
where $x$ is an input, ${\rm spline}(x; \theta)=\sum_i \theta_{i} B_i (x)$ denotes the spline function with learnable coefficients $\theta$, $b(x) = {\rm SiLU}(x) = x/(1 + e^{-x})$ represents an activation function, and $\alpha$ and $\beta$ denote learnable coefficients. Spline functions are piecewise polynomial functions with high expressiveness and can approximate any continuous function. KAN can approximate various complex nonlinear functions by adjusting the parameters and coefficients of the activation function~\cite{liu2024kan}. 
The activation value of the $(l+1,j)$ neuron can be written as
\begin{equation}
    x_{l+1,j}=\sum_{i=1}^{n_l} \tilde{\phi}_{l,j,i}(x_{l,i}),\; j=1,\cdots,n_{l+1},
\end{equation}
where $\tilde{\phi}_{l,j,i}$ denotes the activation function that connects $(l,i)$-neuron and $(l+1,j)$-neuron, $l$ is the index of layers, and $i,j$ is the index of neuron in the $l$-th layer. Then, it can be expressed in matrix form as
\begin{equation}
    {x}_{l+1}=\begin{bmatrix}
        \tilde{\phi}_{l,1,1}(\cdot)&\tilde{\phi}_{l,1,2}(\cdot)& \cdots & \tilde{\phi}_{l,1,n_l}(\cdot)\\
        \tilde{\phi}_{l,2,1}(\cdot)&\tilde{\phi}_{l,2,2}(\cdot)& \cdots & \tilde{\phi}_{l,2,n_l}(\cdot)\\
        \vdots&\vdots&  & \vdots\\
        \tilde{\phi}_{l,n_{l+1},1}(\cdot)&\tilde{\phi}_{l,n_{l+1},2}(\cdot)& \cdots & \tilde{\phi}_{l,n_{l+1},n_l}(\cdot)\\
    \end{bmatrix}{x}_l = \Phi_l {x}_l,
\end{equation}
where $\Phi_l $ denotes the matrix with function elements corresponding to the $l$-th KAN layer. A general KAN network, ${\rm KAN}:\mathbb{R}^{n_0}\to \mathbb{R}$, with $L$ layers can be represented as
\begin{equation} \label{eq:kan_layers}
    {\rm KAN}({x}_{\rm in})= (\Phi_{L-1} \circ \Phi_{L-2} \circ \cdots \circ \Phi_{1} \circ \Phi_{0} ) {x}_{\rm in},
\end{equation}
where ${x}_{\rm in}\in \mathbb{R}^{n_{0}}$ is an input vector. In this work, we train a KAN-based model, $\pi_\theta$, to approximate $\pi^{\ast}$ in~\eqref{eq:true_tsg}.

The coefficients of the spline, $\theta_i$, are updated through the AdamW method~\cite{loshchilov2017decoupled} using the loss function $\mathcal{L}(\theta)$ in~\eqref{eq:log_aug_msrelu}. The update process for the hyperparameters, $\theta^{(q+1)}_{i}=\theta^{(q)}_{i}-\Delta_{lr}\frac{\partial \mathcal{L}}{\partial \theta_{i}}$, where $\Delta_{lr}$ is the learning rate. Additionally, KAN uses a regularization term $\mathcal{R}(\theta)$, which is added to the loss function, to mitigate the overfitting problem, see~\cite{liu2024kan} for further details.

To characterize the approximating properties of KANs, we define the grid corresponding to the grid size parameter, G.
\begin{theorem} \label{thm:KAT} {$\left[\text{Approximation theory~\cite{liu2024kan}} \right]$}
    Suppose that a function, $f(x):\mathcal{X}\to \mathcal{T}$, admits a representation
    \begin{equation}
        f=(\Phi_{L-1} \circ \Phi_{L-2} \circ \cdots \circ \Phi_1 \circ \Phi_0 ) x,
    \end{equation}
    where each $\Phi_{l}$ is $(k+1)$-times continuously differentiable. Given $f$ and its representation, there exists a constant $C$, such that the following approximation bound depending on the grid size, $G$, holds where
    there exists $k$-th order B-spline functions $\Phi^G_l$ such that for any $0\leq m \leq k$, with the bound
    \begin{equation}
        \|f-\left( \Phi^G_{L-1} \circ \Phi^G_{L-2} \circ \cdots \circ \Phi^G_1 \circ \Phi^G_0 \right) x\|_{C^m} \leq CG^{-k-1+m}.
    \end{equation}
    The magnitude of derivatives up to order $m$ is measured by the $C^m-$norm as
    \begin{equation}
        \|g\|_{C^m} = \max_{|\beta|\leq m} \sup_{x\in[0,1]^n}|D^\beta g(x) |.
    \end{equation}    
\end{theorem}

\begin{theorem}
    Given the grid size $G\in \mathbb{N}$, the pointwise approximation error is bounded, i.e.,
    $$\|\Delta_{\pi_{\theta^{\ast}}}\| =\| \pi^{\ast}(x)-\hat{\pi}_{\theta} (x) \| \leq \zeta^{\pi_{\theta}}(G) \in \mathbb{R}^{+},\; \forall x\in \mathcal{X} .$$
    such that
    $$\lim_{G\to \infty} \zeta^{\pi_{\theta}}(G) =0.$$
\end{theorem}
\begin{proof}
    We assume that $\pi^{\ast}(x)$ is a continuous function, whose domain, $\mathcal{X}\subset \mathbb{R}^{n}$, and image set, $\mathcal{T}\subset \mathbb{R}$, are compact, being equivalent to closed and bounded. Suppose an approximated model using KAN with the grid size $G\in \mathbb{N}$, i.e., $\pi_{\theta}(x)={\rm KAN}(x)$ in~\eqref{eq:kan_layers}. Then, $\pi_{\theta}(x)$ is made up of the activation function in~\eqref{eq:residual_act_fxn} that is the summation of the spline function and ${\rm SiLU}(x)$. Since ${\rm SiLU}(x)$ is infinitely continuously differentiable, the condition of Theorem~\eqref{thm:KAT} holds. Therefore, there exists a constant $C$, such that the approximation bound can be written as $\zeta^{\pi_{\theta}}=CG^{-k-1+m}$ for any $0\leq m\leq k$, i.e., $\| \pi^{\ast}(x)-\hat{\pi}_{\theta} (x) \| \leq CG^{-k-1+m}$. 
    Additionally, since $0\leq m\leq k$, $\zeta^{\pi_{\theta}}=CG^{-k-1+m}\leq CG^{-1}$ when $m=k$, and thus $\lim_{G\to \infty} CG^{-1} =0$. 
    % the pointwise approximation error is bounded and $\zeta^{\pi_{\theta}}$ converges zero as $G\to \infty$.
\end{proof}


% We aim to prove that Constraint-informed KAN (CIKAN) as the backbone network can effectively approximate the optimal time shift governor function, $\pi^{\ast}$. Suppose the optimal time shift governor function for taking the time shift parameter $t_{\rm shift}$ with respect to a state $x$ is $(k+1)-$times continuously differentiable, which is represented as $\pi^{\ast}(x)$. Hence, we implements the KAN architecture for the $\pi(x;\theta)=(\Phi_{L-1}\circ \cdots \Phi_0)x$, where each $\Phi_i$ represents a neural network layer.

% Our goal is to find an approximation function $\pi(x;\theta)$ that is as close as possible to $\pi^{\ast}(x)$. Considering the mean squared error in the SINN loss function and $t_{\rm shift}=\pi(x;\theta)$, we have 
% \begin{equation}
%     \mathbb{E}\left[ (\pi(x;\theta)-\pi^{\ast}(x))^2 \right] = \mathbb{E}[ (\pi(x;\theta) - t^{bi}_{\rm shift})^2]+C,
% \end{equation}
% where $C=\mathbb{E}\left[ ( t^{bi}_{\rm shift} - \pi^{\ast}(x) )^2 \right]$ is a constant independent of $\theta$, and $t^{bi}_{\rm shift} $ is computed from the bisection algorithm with an error bound, i.e., $C_{\epsilon}=\max |t^{bi}_{\rm shift}-\pi^\ast(x)|$. Therefore, minimizing the loss function $\mathcal{L}(\theta)$ is equivalent to minimizing the mean squared error between the approximated time shift governor function $\pi(x;\theta)$ and the target value $t^{bi}_{\rm shift}$. 
% Given the grid size $G$, the error is bounded, i.e., $\| \pi(x;\theta)-\pi^{\ast}(x) \|_{C^m} \leq CG^{-k-1+m}\leq C_{\epsilon} G^{-k-1+m}$, following Theorem~\ref{thm:KAT}.
% \clearpage

% \begin{theorem} \label{thm:apprx}
%     Let $\pi(x;\theta)$ be the approximated time shift governor function~\eqref{eq:kan_layers} based on~\eqref{eq:residual_act_fxn}, where the spline functions and the activation function are Lipschitz continuous with Lipschitz constants $L_{\rm spline}$ and $L_{b}$, respectively. Assume that the optimal time shift governor function $\pi^\ast(x)$ is also Lipschitz continuous with Lipschitz constant $L_{\pi^{\ast}}$. Then, for any $\epsilon>0$, there exists a set of parameters $\theta^{\ast}$ such that 
%     \begin{equation}
%         |\pi(x;\theta^\ast)-\pi^\ast (x) | \leq \epsilon,
%     \end{equation}
%     and for any $\theta\in \Theta$,
%     \begin{equation} \label{eq:3}
%         |\pi(x;\theta)-\pi^{\ast}(x)| \leq \epsilon + C\|\theta-\theta^\ast\|_2,
%     \end{equation}
%     where $C=\sqrt{m}(\alpha_{\rm max} L_{\rm spline} + \beta_{\rm max} L_{\rm b})$, $m$ is the number of basis function used in the spline approximation, $\alpha_{\rm max}=\max_i \alpha_i$ and $\beta_{\rm max}=\max_i \beta_i$.
% \end{theorem}
% \begin{proof}
%     By the universal approximation theorem for spline functions~\cite{schumaker2007spline}, $\forall \epsilon>0$, there exists $\theta^\ast$ such that
%     \begin{equation}
%         \| \pi(x; \theta^\ast) - \pi^\ast (x) \|_{\infty} \leq \epsilon.
%     \end{equation}
%     For a function with $1$-D output, $| \pi(x; \theta^\ast) - \pi^\ast (x) |=\| \pi(x; \theta^\ast) - \pi^\ast (x) \|_{\infty}$.
%     Then, for any $\theta \in \Theta$, we have
%     \begin{align} \label{eq:1}
%         | \pi(x; \theta)-\pi^\ast (x) | &\leq | \pi(x; \theta)-\pi(x; \theta^\ast) | + | \pi(x; \theta^\ast)-\pi^\ast (x) | \nonumber \\
%         &\leq | \pi(x; \theta)-\pi(x; \theta^\ast) | +\epsilon.
%     \end{align}
%     % \begin{align} \label{eq:1}
%     %     \| \pi(x; \theta)-\pi^\ast (x) \|_{\infty} &\leq \| \pi(x; \theta)-\pi(x; \theta^\ast) \|_{\infty} + \| \pi(x; \theta^\ast)-\pi^\ast (x) \|_{\infty} \nonumber \\
%     %     &\leq \| \pi(x; \theta)-\pi(x; \theta^\ast) \|_{\infty} +\epsilon.
%     % \end{align}
%     By the Lipschitz continuity of ${\rm spline}(x; \theta)$ and $b(x)$, we obtain
%     \begin{align} \label{eq:2}
%         | \pi(x; \theta) - \pi (x; \theta^\ast) |& \leq  \sum_{i=1}^{m} (\beta_i L_{b} \|\theta_i - \theta_i^\ast\|_2 + \alpha_i L_{\rm spline} \| \theta_i -\theta_i^\ast \|_2 )\nonumber \\
%         &\leq \sqrt{m}(\alpha_{\rm max} L_{\rm spline} +\beta_{\rm max} L_{b} ) \| \theta - \theta^\ast \|_2
%     \end{align}
%     % \begin{align} \label{eq:2}
%     %     \| \pi(x; \theta) - \pi (x; \theta^\ast) \|_{\infty}& \leq \sum_{j\in\{1,\cdots,n-1\}} \sum_{i=1}^{m} (\beta_i L_{b} \|\theta_i - \theta_i^\ast\|_2 + \alpha_i L_{\rm spline} \| \theta_i -\theta_i^\ast \|_2 )\nonumber \\
%     %     &\leq \sqrt{m}(\alpha_{\rm max} L_{\rm spline} +\beta_{\rm max} L_{b} ) \| \theta - \theta^\ast \|_2
%     % \end{align}
%     By substituting \eqref{eq:1} into \eqref{eq:2},
%     \begin{align}
%         | \pi(x; \theta)-\pi^\ast (x) | & \leq \epsilon + | \pi(x; \theta)-\pi(x; \theta^\ast) |  \nonumber\\
%         & \leq \epsilon+ \sqrt{m}(\alpha_{\rm max} L_{\rm spline} +\beta_{\rm max} L_{b} ) \| \theta - \theta^\ast \|_2 = \epsilon + C\| \theta-\theta^\ast \|_2.
%     \end{align}
% \end{proof}
% The proof of Theorem~\eqref{thm:apprx} follows that of~\cite[Theorem 2]{lin2024conflicts}, but is included for clarity purposes.

% \clearpage
% ----- ------ ------ ----- ------ ------ ----- ------ ------ ----- ------ ------ ----- ------ ------ ----- ------ ------ \\
% Suppose $\hat{\pi}_{\theta^{\ast}} $ is a Lipschitz continuous function over ${\rm chull}(\mathcal{X}_{\eta})$.
% \begin{theorem} \label{thm:appx_fxn}
%     The following properties hold:
%     \begin{enumerate}
%         \item $\hat{\pi}_{\theta^{\ast}} (x) \in \mathcal{T}, \forall x \in \mathcal{X} .$
%         \item The pointwise approximation error $\Delta_{\pi_{\theta^{\ast}}}$ of $\hat{\pi}_{\theta^{\ast}} $ is bounded as
%         \begin{align*}
%              \forall x \in \mathcal{X},\; \|\Delta_{\pi_{\theta^{\ast}}}\| =\| \pi^{\ast}(x)-\hat{\pi}_{\theta^{\ast}} (x) \| \leq L \|x-\tilde{x}\| \leq e^{\pi_{\theta^{\ast}}}(x) \leq \zeta^{\pi_{\theta^{\ast}}} = \sup_{x\in \mathcal{X}} e^{\pi_{\theta^{\ast}}}
%         \end{align*}
%         \item $\lim_{\eta\to \infty}\zeta^{\pi_{\theta^{\ast}}}=0.$ {\color{red} pointwise convergence vs uniform convergence}
%     \end{enumerate}    
% \end{theorem}
